OHIE: Blockchain Scaling Made Simple

Many blockchain consensus protocols have been proposed recently to scale the throughput of a blockchain with available bandwidth. However, these protocols are becoming increasingly complex, making it more and more difficult to produce proofs of their security guarantees. We propose a novel permissionless blockchain protocol OHIE which explicitly aims for simplicity. OHIE composes as many parallel instances of Bitcoin's original (and simple) backbone protocol as needed to achieve excellent throughput. We formally prove the safety and liveness properties of OHIE. We demonstrate its performance with a prototype implementation and large-scale experiments with up to 50,000 nodes. In our experiments, OHIE achieves linear scaling with available bandwidth, providing about 4-10 Mbps transaction throughput (under 8-20 Mbps per-node available bandwidth configurations) and at least about 20x better decentralization over prior works.

==> figures/chainDiff.tex <==
\begin{footnotesize}

\begin{figure}[t]
\centering
\pgfplotsset{compat=newest,
legend style={font=\footnotesize},
label style={font=\footnotesize},
tick label style={font=\footnotesize},
title style={font=\footnotesize},
footnotesize,height=6cm,width=0.5\textwidth,
no markers}

\begin{tikzpicture}[scale=0.8]
\begin{axis}[
legend columns=3,
legend entries={max block difference,Max. rank difference},
legend to name=fig:chain-diff-internal,
mark=none,
% title={Block size = 5KB},
ylabel={Max. Difference across chains},
xlabel={Time (sec)},
grid=major,
xtick=\empty, ytick=\empty,
extra x ticks={0,1000,...,5000},
extra y ticks={0, 200,...,1000},
grid=major
]
\addplot table[x=x1,y=y1] {figures/chainDiffData.dat};
\addplot table[x=x1,y=y2] {figures/chainDiffData.dat};
\end{axis}
\end{tikzpicture}
\ref{fig:chain-diff-internal}
\caption{The difference between the number of blocks on the longest
  and shortest chain grows unbounded over time, whereas
  difference between ${\tt rank}$ values in \tool do not. Here, we run
  \codename with $k=16$ chains. 
%  , generating $600$XXXXXX blocks of \blocksize every $10$ seconds. 
  }
\vspace*{-4mm}
\label{fig:chaindiff}
\end{figure}
\end{footnotesize}


==> figures/code.tex <==

\begin{figure*}
\begin{subfigure}{.35\textwidth}
\pgfplotsset{compat=newest,
legend style={font=\footnotesize},
label style={font=\footnotesize},
tick label style={font=\footnotesize},
title style={font=\footnotesize}}
\centering\captionsetup{width=.8\linewidth}
\begin{framed}
\footnotesize
\begin{algorithmic}[1]
\State $d \leftarrow \log_2 (\frac{1}{kp})$; %\Comment{PoW difficulty}
\State $V_i \leftarrow$ \{(genesis block of chain $i$, the attachment for genesis block of chain $i$)\}, for $0\le i\le k-1$;
\State $M \leftarrow $ Merkle tree of the hashes of the $k$ genesis blocks;
%MMM// modelled as ${\tt H2.compute}(B)$
\label{code:h2computeinitial}
\State ${\tt trailing}$ $\leftarrow $ hash of the genesis block of chain $0$;
\State
\State {\sc Ohie}() \{
\State \hspace*{2mm}{\bf repeat forever}
\State \hspace*{8mm}ReceiveState(); \label{code:mainloop1}
\State \hspace*{8mm}Mining();
\State \hspace*{8mm}SendState(); \label{code:mainloop2}
\State \}
\State
\State Mining() \{
\State \hspace*{2mm}$B.{\tt transactions} \leftarrow$ getTX();
\State \hspace*{2mm}$B.{\tt root}$ $\leftarrow$ root of Merkle tree $M$;
\State \hspace*{2mm}$B.{\tt trailing} \leftarrow$ ${\tt trailing}$;
\State \hspace*{2mm}$B.{\tt nonce} \leftarrow$  new\_nonce();
\State \hspace*{2mm}$\widehat{B}.{\tt hash} \leftarrow hash(B)$;
%MMM// modelled as ${\tt H1.compute}(B)$
\label{code:h1compute}
\State \hspace*{2mm}{\bf if} ($\widehat{B}.{\tt hash}$ has $d$ leading zeroes) \{
\State \hspace*{4mm}$i$ $\leftarrow$ last $\log_2 k$ bits of $\widehat{B}.{\tt hash}$;
\State \hspace*{4mm}$\widehat{B}.{\tt leaf} \leftarrow$ leaf $i$ of $M$;
\State \hspace*{4mm}$\widehat{B}.{\tt leaf\_proof} \leftarrow M$.MerkleProof($i$);
\State \hspace*{4mm}ProcessBlock($B$, $\widehat{B}$);
\State \hspace*{2mm}\}
\State \}
\end{algorithmic}
\normalsize
\end{framed}
\end{subfigure}
%
\begin{subfigure}{.34\textwidth}
\pgfplotsset{compat=newest,
legend style={font=\footnotesize},
label style={font=\footnotesize},
tick label style={font=\footnotesize},
title style={font=\footnotesize}}
\centering\captionsetup{width=.9\linewidth}
\begin{framed}
\footnotesize
\begin{algorithmic}[1]
\setcounter{ALG@line}{25}
\State ProcessBlock($B$, $\widehat{B}$) \{
\State \hspace*{2mm}$i$ $\leftarrow$ last $\log_2 k$ bits of $\widehat{B}.{\tt hash}$;
\State \hspace*{2mm}verify $\widehat{B}.{\tt hash}$ has $d$ leading zeroes;
\State \hspace*{2mm}verify that $hash(B) = \widehat{B}.{\tt hash}$;
%MMM// modelled as ${\tt H1.verify}(B, \widehat{B}.{\tt hash})$;
\label{code:h1verify}
\State \hspace*{2mm}verify that $\widehat{B}.{\tt leaf}$ is leaf $i$ in the Merkle tree, based on $B.{\tt root}$ and $\widehat{B}.{\tt leaf\_proof}$;
%MMM// modelled as ${\tt H2.verify}()$ invocations
\label{code:h2verify}
\State \hspace*{2mm}verify that $\widehat{B}.{\tt leaf} = \widehat{A}.{\tt hash}$ for some block $(A, \widehat{A}) \in V_i$;
\State \hspace*{2mm}verify that $B.{\tt trailing} = \widehat{C}.{\tt hash}$ for some
block $(C, \widehat{C}) \in \cup_{j=0}^{k-1}V_j$;
\State \hspace*{2mm}{\bf if} (any of the above 5 verifications fail) {\bf then return};
\State
\State \hspace*{2mm}$\widehat{B}.{\tt rank} \leftarrow \widehat{A}.{\tt next\_rank}$;
\label{code:rankstart}
\State \hspace*{2mm}$\widehat{B}.{\tt next\_rank} \leftarrow \widehat{C}.{\tt next\_rank}$;
\State \hspace*{2mm}{\bf if} ($\widehat{B}.{\tt next\_rank}\le \widehat{B}.{\tt rank}$) {\bf then}
\State \hspace*{6mm}$\widehat{B}.{\tt next\_rank}\leftarrow \widehat{B}.{\tt rank}+1$;
\label{code:rankend}
\State
\State \hspace*{2mm}$V_i \leftarrow V_i \cup \{(B, \widehat{B})\}$;
\State \hspace*{2mm}update ${\tt trailing}$;
\State \hspace*{2mm}update Merkle tree $M$;
\label{code:h2compute}
%MMM// modelled as ${\tt H2.compute}()$ invocations
\State \}
\State
\State SendState() \{
\State \hspace*{2mm} send $V_i$ ($0\le i\le k-1$) to other nodes;
\State \hspace*{2mm} // In implementation, only need to send those blocks not sent before.
\State \}
\end{algorithmic}
\normalsize
\end{framed}
\end{subfigure}
%
\begin{subfigure}{.32\textwidth}
  \pgfplotsset{compat=newest,
    legend style={font=\footnotesize},
    label style={font=\footnotesize},
    tick label style={font=\footnotesize},
    title style={font=\footnotesize}}
  \centering\captionsetup{width=.9\linewidth}
  \begin{framed}
    \footnotesize
    \begin{algorithmic}[1]
\setcounter{ALG@line}{48}
\State ReceiveState() \{
\State \hspace*{2mm} {\bf foreach} $(B, \widehat{B})\in$ received state {\bf do} \State \hspace*{6mm} ProcessBlock($B$, $\widehat{B}$);
\State // Note that a block $B_1$ should be processed before $B_2$, if $\widehat{B_2}.{\tt leaf}$ or $\widehat{B_2}.{\tt trailing}$ points to $B_1$.
\State \}
\State
      \State OutputSCB() \{
      \State \hspace*{2mm}{\bf for} ($i=0$; $i < k$; $i$++) \{
      \State \hspace*{4mm}$W_i$ $\leftarrow$ getLongestPath($V_i$);
      \State \hspace*{4mm}${\tt partial}_i$ $\leftarrow$ blocks in $W_i$ except the last $T$ blocks;
      \State \hspace*{4mm}($B_i$, $\widehat{B_i}$)  $\leftarrow$ the last block in ${\tt partial}_i$;
      \State \hspace*{4mm}$y_i\leftarrow \widehat{B_i}.{\tt next\_rank}$;
      \State \hspace*{2mm}\}
      \State \hspace*{2mm}${\tt confirm\_bar} \leftarrow \min_{i=0}^{k-1} y_i$;
      \State \hspace*{2mm}${\tt all\_par}$ $\leftarrow$ $\cup_{i=0}^{k-1} {\tt partial_i}$;
      \State
      \State \hspace*{2mm}$L \leftarrow \emptyset$; \Comment{fully-confirmed blocks}
      \State \hspace*{2mm}{\bf foreach} $(B,\widehat{B})\in {\tt all\_par}$ \{
      \State \hspace*{4mm}{\bf if} ($\widehat{B}.{\tt rank} < {\tt confirm\_bar}$)
      \State \hspace*{4mm}{\bf then} $L \leftarrow L \cup \{(B, \widehat{B})\}$;
      \State \hspace*{2mm}\}
      \State \hspace*{2mm}sort blocks in $L$ by ${\tt rank}$, tie-breaking favoring smaller chain id;
      \State \hspace*{2mm}{\bf return} $L$;
      \State \}
    \end{algorithmic}
    \normalsize
  \end{framed}
%  \noindent
\end{subfigure}
%
\vspace*{2mm}
\caption{Pseudo-code of the $(k, p, \lambda, T)$-\tool protocol.
%A genesis block $B$ will always have $\widehat{B}.{\tt rank}=0$, $\widehat{B}.{\tt next\_rank}=1$, and $\widehat{B}.{\tt leaf}=\widehat{B}.{\tt leaf\_proof}={\tt null}$.
}
%Parameters $k$ and $T$
%  are fixed values, and are initialized once at the time of
%  deployment.  Similar to Nakamoto consensus, $p$ is dynamically
%  adjusted based on the mining power (not shown).}
\label{fig:code}
\vspace*{-3mm}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> figures/confirmation.tex <==
\begin{tikzpicture}[trim axis left,trim axis right,scale=0.6]
\begin{axis}[
%legend columns=3,
legend columns=3,
legend entries={added;, partial;, full},
legend to name=fig:confirm_internal,
ylabel={Delay (sec)},
xlabel={Available Bandwidth (Mbps)},
nodes near coords,
grid=major
]
  \addplot[
    color=blue,
    mark=square,
  ]
  coordinates {(8,2.81) (12,2.73) (16,2.69) (20,2.64)};
  \addplot[
    color=red,
    mark=*,
  ]
  coordinates {(8,306.3) (12,300.8) (16,300.1) (20,302.4)};
  \addplot[
    color=black,
    mark=x,
  ]
  coordinates {(8,501.4) (12,490.2) (16,500.6) (20,511.3)};
\end{axis}
\end{tikzpicture}
\\
\ref{fig:confirm_internal}
\caption{(Macro experiments) The avg. delay for all nodes to (a)
  add the block to some chain, (b) partially confirm it, and (c)
  fully-confirm it, from the time it is broadcast ($T=30$). 
%
% Delay remains constant with increasing available bandwidth (and
% throughput).
% 
%   confirmation blocks. Delay remain nearly constant with
%   increasing available bandwidth .
}
\label{fig:confirm-30}

